A Software Engineering Perspective on Testing Large Language Models: Research, Practice, Tools and Benchmarks

Large Language Models (LLMs) are rapidly becoming ubiquitous both as stand-alone tools and as components of current and future software systems. To enable usage of LLMs in the high-stake or safety-critical systems of 2030, they need to undergo rigorous testing. Software Engineering (SE) research on testing Machine Learning (ML) components and ML-based systems has systematically explored many topics such as test input generation and robustness. We believe knowledge about tools, benchmarks, research and practitioner views related to LLM testing needs to be similarly organized. To this end, we present a taxonomy of LLM testing topics and conduct preliminary studies of state of the art and practice approaches to research, open-source tools and benchmarks for LLM testing, mapping results onto this taxonomy. Our goal is to identify gaps requiring more research and engineering effort and inspire a clearer communication between LLM practitioners and the SE research community.

==> sections/mapping.tex <==
% THIS FILE IS DEPRECATED

% \sinclair{from here on out in this section, I'm not sure what to include, a lot of it feels like sample text}

%\caroline{(addressed by sinclair) you discussed topics that are out of scope, I think they don't need their own subsection, having discussions only about what exists might be enough here. Then in the end, we can mention all the topics not covered by existing tool and say they are future directions.}
%\red{NOTE to Sinclair: this paper has a taxonomy for LLM evaluation: https://arxiv.org/pdf/2307.03109.pdf (figure 1)}
%     \item What's done in ML but not in LLM
%     \item what's done in LLM but not in ML (expand this taxonomy, check observations)
%     \item what are the future directions and the challenges pursuing them
%     \item threats to validity
%   \subsection{Testing workflow (how to test)}
%       \subsubsection{Test input generation}
%       % Confusingly, they call this "dataset generation"
%       Promptfoo has implemented a CLI tool that will take a YAML file of tests and output more, similar tests, to increase the side of the test suite. They also offer simple methods to create all possible pairwise tests given a few lists. For example, testing french-english, english-spanish, spanish-french, english-french ... translations of the same few equivalent phrases \cite{promptfoo}.
%       Apart from that, test generation remains underexplored.
%       \subsubsection{Test oracle generation and idenfitication}
%       TODO address test oracle identification as well. 
%       We have lots to talk about, including LLM-RAG as judge, LLM as judge, regex, embedding similarity, all as proxy oracles. I discussed this initially in correctness, might need to refactor.
%       \subsubsection{Test adequacy evaluation}
        % Test adequacy evaluation aims to discover whether the
        % existing tests have a good fault-revealing ability. It provides
        % an objective confidence measurement on testing activities.
        % The adequacy criteria can also be adopted to guide test
        % generation. Popular test adequacy evaluation techniques
        % in traditional software testing include code coverage and
        % mutation testing, which are also adopted in ML testing.
%       Current notions of mutation testing or coverage remain under-explored in open-source toolkits. The toolkits often focus on tests that support models hidden behind an API (immutable), and simply encourage the creation of specific benchmarks to evaluate specific functionalities of the LLM.
%       \subsubsection{Test prioritization and reduction}
%       No infrastructure exists for test prioritization and reduction inthe surveyed LLM evaluation toolkits.
%       However, promptfoo does implement caching of test results; if the prompt and model are the same, the generated output will be the same (when deterministic decoding is used). Caching is extremely valuable considering the high compute cost associated with the inference of LLMs \cite{promptfoo}. \caroline{I think caching isn't exactly test reduction}
%       \subsubsection{Bug report analysis, debug and repair}
%       Bug report analysis, as well as debug and repair, are somewhat out of scope for open-source toolkits dedicated to testing LLMs. 
        % \subsubsection{Debug and repair}
%   \subsection{Testing components (where to test)}
%       \subsubsection{Data testing}
%       Data testing is underexplored in open-source toolkits, with no attention being given to validating that the data is correct.
%       This could be because the data is assumed to be clean, and that LLM training is self-supervised in nature, meaning that validating the labels are correct isn't required. Still, undesirable text in a training dataset can introduce bugs in the resulting LLM model.
%       More development is required to round out data testing using open-source toolkits, both for fine-tuning and for RAG knowledge-bases.
%       DeepEval does implement a few LLM-as-judge tests that assess the retriever's outputs exclusively, in a RAG pipeline. These tests could be used to verify that the data in the knowledge base is indeed accurate, however the retriever could also fail to retrieve erroneous documents, leaving the data bug undetected.
%       \subsubsection{Learning program testing}
%       No open-source toolkit studied explores learning program testing, largely because very few provide or expect practitioners to fine-tune models.
%       \subsubsection{Framework testing}
%       Framework testing is out of scope for the studied toolkits, and they aim to be framework agnostic, assuming LLMs accept a string as input and a string as output.
%   \subsection{Testing properties (what to test)}
%       \subsubsection{Correctness}
%       Correctness testing is traditionally addressed using hold-out cross validation, a "test set" targeting some desired functionality.
%       Indeed, many benchmark datasets exist for LLM evaluation, aggregated in repositories such as BigBench \cite{bigbench} and OpenAI evals \cite{openaievals}.
%       % These repositories are a composition of multiple individual test sets, each one dedicated to testing different functionality. They provide a common interface for all these test sets, allowing for correctness testing in many different applications.
%       However, the nature of LLMs makes testing for correctness more difficult, in multiple ways.
%       Since practitioners are often not involved with the training process of these models, and with that data being hidden, it is difficult to be certain that these test-sets are indeed "held-out".
%       Since LLMs output open-ended text, outputs can be correct or incorrect in multiple different ways.
%       A response that isn't an exact match to the "ground truth" isn't necessarily incorrect; it could simply be worded differently.
%       Most other ML systems are correct or incorrect in a quantitative way, such as the mean squared error of a regression model being too high, or by producing incorrect classifications.
%       With open-ended text, the notion of "correct" can be difficult to define and quantify.
%       In a medical or trivia setting, correctness can be quite objective.
%       However, in a setting such as customer service, an impolite response could be considered incorrect.
%       In other words, the content, the perceived tone, and the delivery of the response factor into determining if the generated output is "correct". 
%       LLMs have a uniquely challenging "oracle problem", and most LLM evaluation toolkits studied provide numerous tests to address this challenge. 
%       Often an LLM is used as an evaluator, to evaluate subjective properties of the response such as "conciseness", "relevance", and "coherence".
%       For cases where correctness hinges on factual information, LLMs can again be used to verify if the output is "similar" to a provided, ideal response.
%       This evaluator LLM can optionally be augmented with a knowledge base of factual information, in a RAG system.
%       Additionally, tests that are regular expressions can be used to identify if responses include specific correct or incorrect information.
%       It should be noted that while there has been a lot of engineering effort dedicated to addressing this oracle problem and assessing the correctness of generated outputs, the problem is far from solved and there is no universal solution to testing LLMs for correctness.
%       % A lot of open source stuff works on this, with RAG and with LLM-as-a-judge
%       \subsubsection{Model relevance}
%       % poor model relevance is overfitting or underfitting.
%       % TODO address the fact that I can't find anything on this topic in the open-source body of work. Nothing about testing for overfitting or underfitting, again because we're sort of not concerned about that with the scale of the data and the size of the model.
%       % Or because even if open-source could test this, they wouldn't be able to do anything about it.
%       Model relevance is often assessed via benchmark datasets, as seen in OpenAI evals, OpenCompass, and other benchmarks. Many benchmarks exist, creating test sets for very specific functionality, assessing the model's relevance to that subsets of data.
%       However, very little tooling exists further to assess model relevance, apart from resources that seek to benchmark LLMs on as many tasks as possible, and aggregate the results.
%       \subsubsection{Robustness and security}
%       % Robustness. Robustness studies the stability of a system when facing unexpected inputs.
%  Specifically, out-of-distribution (OOD) [207 ] and adversarial robustness are two popular research
% topics for robustness. 
% Security: the system's resilience against potential harm, danger, or loss made via manipulating or illegally accessing ML components.
%           Security in LLMs is difficult to achieve, because LLMs are largely black-box, and the user can often prompt the model freely using text.
%           Giskard \cite{giskard} has implemented a "control character invariance test", where models are evaluated based on their ability to ignore control characters and whitespace appended to the input.
%           Giskard has also implemented a "Binary Cohesion test", where given two similar inputs, the test is passed if the outputs are judged to be the same according to an LLM.
%           
%           TruLens Eval implements a test that uses a Named Entity Recognition (NER) model to detect Personally Identifiable Information (PII). This could be used to verify security against adversarial prompts that aim to uncover PII from the training set, if any.
%           This test is critical, especially considering that most LLM practitioners cannot verify that the training data of the LLM doesn't contain sensitive information.
%           Though not specifically motivated by robustness, a correctness test for concrete properties of an LLM's response could be used to test security and robustness. For example, almost all toolkits could be used to create an LLM-as-judge test with the requirement that "the model should refuse to answer", when the prompt attempts to extract sensitive information  or attempts a "prompt injection" \cite{TODO prompt_injection}.
%       \subsubsection{Efficiency}
%       % Again, couldn't find something in the literature addressing this. 
%       % This is more about training speed, and efficiency.
%       Efficiency in inference is a large concern for practitioners using open-source toolkits. Inference time significantly impacts user experience \cite{msftLLM}, and high generation costs scale with the generated output length (billing is often per-token).
%       Most toolkits provide a very simple test to assert that the inference time or cost of a generation is below a certain threshold, and there is little functionality provided past those very basic tests.
%       \subsubsection{Fairness}
%       DeepEval implements a very basic test of Fairness, by asking an LLM if the string under test contains a biased opinions or not.
%       This test is called the "bias metric", and quite rudimentary. 
%       % NOTE I've seen this evaluated, in the literature, by looking at the outputted probabilities and comparing them for male vs female pronouns, for example. I haven't seen such a test implemented in open source however.
%       \subsubsection{Interpretability}
%       While most of the open-source toolkits treat LLMs as a black-box, Langchain has attempted to test the interpretability of an LLM agent via a "Trajectory Evaluation".
%       This test feeds an agent's steps towards completing a task to another LLM.
%       That LLM judges whether or not the agent accomplished the problem well. In a sense, it is attempting to test that the sequence of steps towards the goal is interpretable. However, the process of generating those individual steps remains a black-box.
%       % NOTE this is a higher level than traditional 
%       
%       \subsubsection{Privacy}
%       % ML system's ability to preserve private data information. Differential privacy, usually applied to Training data.
%       Testing for data privacy appears to be a large gap in available open-source tooling.
%       Concepts such as differential privacy are typically only applicable to training data, and as previously stated, practitioners rarely have the means to train LLMs themselves.
%       However, there are still potential concerns for privacy, including data introduced via a knowledge base for retrieval-augmented generation (RAG) or during Fine-tuning.
%       Certain adversarial prompts can be used to extract original training data with high efficiency \cite{training_data_extraction}, a principle privacy concern.
%       Much further work and testing methodology is needed to verify that LLMs can keep their data private.
%   
%   \subsection{Application Scenario}
%       \subsubsection{Machine translation}
%       Machine Translation has the benefit of being a relatively mature area of research, with benchmarks and metrics such as BLEU score \cite{}.
%       The frameworks TODO, TODO, TODO implement BLEU within their library, enabling LLMs to easily be tested as translators.
%       However, evaluating Machine Translation systems is far from "solved". Multiple newer metrics have been proposed \cite{METEOR} \cite{COMET}, \cite{TER (translation error rate)} largely targetting a high correlation between metric output and human preference and professional evaluation.
%       Practitioners could also construct an LLM-as-a-judge test that asks a language model to assess how accurate, fluent, and cohesive a certain translation is.
%       \subsubsection{Natural language inference}
%       Natural Language Inference (NLI) is not addressed in any of the studied open-source toolkits.


%       \caroline{are there more LLM specific applications? like chatbot etc.? did any of the tools mention this?}

==> sections/threats_to_validity.tex <==
\section{Threats To Validity}
\label{sec:threats}
\green{In each section note the scope of each section and at the end note what we could have done instead; threats to validity with conclusion; include a name for each section that corresponds the threats to validity}
To motivate our vision for 2030, we provided a brief overview of research literature relating to testing LLMs, and a survey of a few open-source tools, and a preliminary analysis of online community discourse.
With publications relating to LLMs growing exponentially, it's difficult to conduct a comprehensive literature review, and be confident that it is complete.
Future research should increase the scope of the open-source analysis and literature review, to bolster claims about the strengths and gaps  of both bodies of work.
The survey of open-source tooling dedicated to LLMs is far from comprehensive, with only 8 tools studied, posing a risk that important tools were ommitted from the analysis.
Additionally, the analysis of tooling relies exclusively on documentation, which may reveal less when compared to dedicated experimentation and code review.
